GLUE: Coordinating Pre-Trained Generative Models for System-Level Design

Engineering complex systems (aircraft, buildings, vehicles) requires coordinating geometric and performance couplings across subsystems. As generative models proliferate for specialized domains, a key research gap is how to coordinate frozen, pre-trained submodels to generate full-system designs that are feasible, diverse, and high-performing. We introduce GLUE, which orchestrates pre-trained, frozen generators while enforcing system-level feasibility, optimality, and diversity. Compatible models must be end-to-end differentiable with a smooth, well-behaved latent-to-output mapping. We propose and benchmark (i) data-driven GLUE models trained on pre-generated system-level designs and (ii) a data-free GLUE model trained on a differentiable geometry layer. On a UAV design problem with five coupling constraints, we find that data-driven approaches yield diverse, high-performing designs but require large datasets to satisfy constraints reliably. The data-free approach is competitive with Bayesian optimization and gradient-based optimization in performance and feasibility while training a full generative model in only ~10 min on an RTX 4090 GPU, requiring more than two orders of magnitude fewer geometry evaluations and FLOPs than the data-driven method. We identify equality constraint satisfaction as a key difficulty and remaining limitation, and ablate approaches that improve this for the data-free approach. As a first step toward scaling generative design to complex, real-world engineering systems, this work explores how unmodified, domain-informed submodels can be integrated into a modular generative workflow.

==> figures/jm-alm-comparison/case_1_b/alm-vs-manual_table.tex <==
\begin{tabular}{lrrrrrr}

 & C\_bb & C\_box\_pl & C\_di\_tol & C\_wx\_tol & C\_lift\_tol & All Satisfied \\
\midrule
HC-ALM & \textbf{100}\% & 97.7\% & 77.0\% & 93.3\% & 87.7\% & \textbf{60.7\%} \\
pooled ALM & \textbf{100}\% & 98.7\% & 74.3\% & 89.7\% & 92.3\% & \textbf{58.7\%} \\
Manual Const. & \textbf{100}\% & 93.7\% & 72.0\% & 97.7\% & 85.3\% & \textbf{55.0\%} \\
Manual Ramp & \textbf{100}\% & 91.0\% & 70.7\% & 97.3\% & 87.0\% & \textbf{53.7\%} \\
\bottomrule
\end{tabular}


==> nomenclature.tex <==
\section*{Nomenclature}
\addcontentsline{toc}{section}{Nomenclature}

\subsection*{Spaces and Dimensionality}
\begin{tabbing}
\hspace{3cm} \= \kill
$\mathcal{Z}$ \>  Unified subsystem latent space \\
$\mathcal{Z}_i$ \> Latent space for subsystem $i$ \\
$\mathcal{X}$ \> Design parameter space \\
$\mathcal{X}_i$ \> Design parameter space for subsystem $i$ \\
$d_i$ \> Latent dimensionality for subsystem $i$ \\
$D$ \> Number of features/dimensions in data \\
\end{tabbing}

\subsection*{Latent Codes and Design Parameters}
\begin{tabbing}
\hspace{3cm} \= \kill
$\zeta$ \> System-level latent code \\
$z_W$ \> Wing latent codes \\
$z_F$ \> Fuselage latent code \\
$z_I$ \> Internals latent code \\
$z$ \> Generic latent code \\
$x_C$ \> Coupling variables \\
$x_F$ \> Fuselage geometric parameters \\
$x_W$ \> Wing geometric parameters \\
$x_I$ \> Internals placement parameters \\
$\mathbf{x}$ \> Complete design parameters \\
\end{tabbing}

\subsection*{Models and Functions}
\begin{tabbing}
\hspace{3cm} \= \kill
$S_i$ \> Subsystem model $i$ \\
$\Phi$ \> \ac{GLUE} model \\
$\theta_\Phi$ \> \ac{GLUE} model parameters \\
$\mathcal{G}$ \> Differentiable geometry layer \\
$Q$ \> Q-Network for mutual information \\
$\mathcal{B}(u,v)$ \> Bicubic Bézier surface \\
$B_i^3(t)$ \> Cubic Bernstein polynomial \\
\end{tabbing}

\subsection*{Objectives and Constraints}
\begin{tabbing}
\hspace{3cm} \= \kill
$\Omass$ \> Mass objective \\
$O_d$ \> Drag objective \\
$n_o$ \> Number of objectives \\
$n_c$ \> Number of constraints \\
$\Clift$ \> Lift constraint \\
$\Cwx$ \> Wing placement constraint \\
$\Cdi$ \> Dihedral angle constraint \\
$\Cbb$ \> Bounding box constraint \\
$\Cboxpl$ \> Box placement constraint \\
$\langle C_K \rangle$ \> Average constraint violation \\
\end{tabbing}

\clearpage
\subsection*{Mass and Structural Parameters}
\begin{tabbing}
\hspace{3cm} \= \kill
$m_{\text{wing}}$ \> Wing mass \\
$m_{\text{fuselage}}$ \> Fuselage mass \\
$m_{\text{cargo}}$ \> Cargo/payload mass \\
$M_{\text{root}}$ \> Root bending moment \\
$\alpha_w$ \> Wing mass scaling constant \\
$\alpha_f$ \> Fuselage mass scaling constant \\
$g$ \> Gravitational acceleration \\
\end{tabbing}

\subsection*{Aerodynamic Parameters}
\begin{tabbing}
\hspace{3cm} \= \kill
$V$ \> Flight velocity \\
$h_{\text{alt}}$ \> Altitude \\
$\rho$ \> Air density \\
$\mu$ \> Dynamic viscosity \\
$c$ \> Wing chord \\
$b$ \> Wing span \\
$L$ \> Lift force \\
$L_{\text{required}}$ \> Required lift \\
$L_{\text{supplied}}$ \> Supplied lift \\
$L_1, L_2$ \> Lift from front/rear wing \\
$C_L$ \> Coefficient of lift (finite wing) \\
$C_\ell$ \> Sectional lift coefficient (airfoil) \\
$Re$ \> Reynolds number \\
$AR$ \> Aspect ratio \\
$e$ \> Oswald efficiency factor \\
$L/D$ \> Lift-to-drag ratio \\
\end{tabbing}

\subsection*{Geometric Parameters}
\begin{tabbing}
\hspace{3cm} \= \kill
$\Gamma_{\text{wing}}$ \> Wing dihedral angle \\
$\Gamma_{\text{fuselage}}$ \> Fuselage interface dihedral angle \\
$a_{bb}, b_{bb}$ \> Bounding box dimensions \\
$\ell, w, h_{\text{box}}$ \> Box length, width, height \\
$\mathcal{V}$ \> Volume \\
$\mathcal{V}_i$ \> Volume of box $i$ \\
$S$ \> Surface area \\
$A_f$ \> Frontal area \\
$\delta$ \> Safety margin \\
$d_{j,k}$ \> Signed distance from point to surface \\
$\kappa$ \> Curvature \\
\end{tabbing}


\subsection*{VAE Parameters}
\begin{tabbing}
\hspace{3cm} \= \kill
$\boldsymbol{\mu}_{\text{enc}}$ \> VAE encoder mean output \\
$\boldsymbol{\sigma}^2_{\text{enc}}$ \> VAE encoder variance output \\
$\boldsymbol{\epsilon}$ \> Random noise vector \\
\end{tabbing}

\clearpage

\subsection*{Bézier Surface Parameters}
\begin{tabbing}
\hspace{3cm} \= \kill
$u, v$ \> Surface parameters \\
$t$ \> Curve parameter \\
$\mathbf{P}_{ij}$ \> Bézier control points \\
$M$ \> Bézier basis matrix \\
$n$ \> Tessellation resolution \\
$\mathbf{p}$ \> Query point \\
$\mathbf{o}$ \> Interior origin point \\
$\mathbf{d}$ \> Ray direction vector \\
$\mathbf{n}$ \> Normal vector \\
\end{tabbing}

\subsection*{Loss Functions and Weights}
\begin{tabbing}
\hspace{3cm} \= \kill
$\mathcal{L}_{\text{total}}$ \> Total loss function \\
$\mathcal{L}_{\text{DPP}}$ \> Determinantal point process loss \\
$\mathcal{L}_{\text{PA-DPP}}$ \> Performance-augmented DPP loss \\
$\mathcal{L}_{\text{recon}}$ \> Reconstruction loss \\
$\mathcal{L}_{\text{KL}}$ \> Kullback-Leibler divergence loss \\
$\mathcal{L}_{\text{MI}}$ \> Mutual information loss \\
$\lambda_k$ \> Lagrange multipliers for constraints \\
$\lambda_{\text{perf}}$ \> Performance loss weight \\
$\lambda_{\text{DPP}}$ \> DPP diversity weight \\
$\lambda_{\text{MI}}$ \> Mutual information weight \\
$\beta_{\text{KL}}$ \> KL divergence weight \\
\end{tabbing}

\subsection*{DPP (Determinantal Point Process)}
\begin{tabbing}
\hspace{3cm} \= \kill
$\mathbf{K}$ \> Similarity kernel matrix \\
$K_{ij}$ \> Kernel matrix element \\
$\mathbf{L}$ \> Regularized kernel matrix \\
$\mathbf{q}$ \> Quality score vector \\
$q_i$ \> Quality score for sample $i$ \\
$\sigma_{\text{DPP}}$ \> Kernel length scale \\
$d(\mathbf{x}_i, \mathbf{x}_j)$ \> Distance between samples \\
\end{tabbing}

\subsection*{ALM (Augmented Lagrangian Method)}
\begin{tabbing}
\hspace{3cm} \= \kill
$\mathbf{c}_t$ \> Constraint violations at epoch $t$ \\
$\boldsymbol{\lambda}_t$ \> Lagrange multipliers at epoch $t$ \\
$\boldsymbol{\mu}_t$ \> ALM penalty parameters at epoch $t$ \\
$\alpha$ \> Momentum parameter \\
$\gamma$ \> ALM growth rate \\
$\epsilon$ \> Small constant for numerical stability \\
$T_{\text{warmup}}$ \> Number of warmup epochs \\
$\mathbf{v}_t$ \> Adaptive gradient accumulator \\
$K$ \> Number of constraints \\
\end{tabbing}

\clearpage

\subsection*{Training and Optimization}
\begin{tabbing}
\hspace{3cm} \= \kill
$B_{\text{batch}}$ \> Batch size \\
$t$ \> Timestep or iteration index \\
$\eta$ \> Learning rate \\
$\tau$ \> Temperature parameter \\
$\mathbf{I}$ \> Identity matrix \\
$\odot$ \> Element-wise multiplication \\
\end{tabbing}



==> tables/ablation_SN.tex <==
\begin{table*}[h!]
\centering
\caption[\acl{SN} ablation study for \ac{DF}-\ac{GLUE}]{\acl{SN} ablation study for \ac{DF}-\ac{GLUE}. Without \ac{SN}, equality constraint satisfaction ($\Cwx$, $\Cdi$, $\Clift$) is near zero regardless of whether an inner optimizer is used. With \ac{SN}, feasibility improves markedly. DPP on $\mathcal{X}_\text{vis}$ (6-D) with $\sigma_{\text{DPP}} = 0.5$. IO = Inner optimizer, SN = \acl{SN}.}
\label{tab:sn_ablation_compact}
\footnotesize
\begin{tabular}{c c c c c c c c c c c}
\toprule
SN & IO & $\Omass$ ($\downarrow$) & $\Cwx$ ($\uparrow$) & $\Cdi$ ($\uparrow$) & $\Clift$ ($\uparrow$) & $\Cbb$ ($\uparrow$) & $\Cboxpl$ ($\uparrow$) & Feas. ($\uparrow$) & $\mathrm{DPP}$ ($\downarrow$) \\
\midrule
\xmark & No  & 8.52 & 0.5\% & 0.2\% & 23.1\% & 83.7\% & 78.1\% & 0.0\% & \textbf{3668} \\
\xmark & Yes & 11.9 & 0.0\% & 0.1\% & 3.4\% & 96.9\% & 93.2\% & 0.0\% & \textbf{3677} \\
\cmark & No  & \textbf{2.36} & \textbf{98.4} \% & 66.8\% & 94.7\% & \textbf{100\%} & \textbf{96.8\%} & 60.8\% & 3840  \\
\cmark & Yes & \textbf{2.36} & 98.1\% & \textbf{73.8\%} & \textbf{95.1\%} & \textbf{100\%} & 94.9\% & \textbf{65.9\%} & 3798 \\
\bottomrule
\end{tabular}%
\end{table*}
